Yuga: Automatically Detecting Lifetime Annotation Bugs in the Rust Language

The Rust programming language is becoming increasingly popular among systems programmers due to its efficient performance and robust memory safety guarantees. Rust employs an ownership model to ensure this guarantee by allowing each value to be owned by only one identifier at a time. Additionally, it introduces the concept of borrowing and lifetimes to enable other variables to borrow the values under certain conditions temporarily. Despite its benefits, security vulnerabilities have been reported in Rust projects, often attributed to the use of "unsafe" Rust code. These vulnerabilities, in part, arise from incorrect lifetime annotations on function signatures. However, existing tools fail to detect these bugs, primarily because such bugs are rare, challenging to detect through dynamic analysis, and require explicit memory models. To overcome these limitations, first, we characterize incorrect lifetime annotations as a source of memory safety bugs and leverage this understanding to devise a novel static analysis tool, Yuga, to detect potential lifetime annotation bugs. Yuga uses a multi-phase analysis approach, starting with a quick pattern-matching algorithm to identify potential buggy components and then conducting a flow and field-sensitive alias analysis to confirm the bugs. We also curate new datasets of lifetime annotation bugs. Yuga successfully detects bugs with good precision on these datasets, and we make the code and datasets publicly available for review.

==> sections/biosketches.tex <==
\section*{Author Biosketches}
\thispagestyle{empty}
\addtocounter{page}{-1}
\vspace{-600pt}
\begin{table}[H]
    \begin{tabular}{p{0.2\textwidth} p{0.7\textwidth}}
        \raisebox{-0.92\totalheight}[0pt][\totalheight]{\includegraphics[width=0.4\columnwidth]{figures/vikram.jpg}} & 
        Vikram Nitin is a PhD student at Columbia University, advised by Prof. Baishakhi Ray. His research focuses on modernization of legacy software applications, through techniques like re-partitioning monolithic applications as microservices, and converting code from older programming languages to more modern ones. Of late, he has been interested in building tools and systems for the Rust programming language. \\
        \raisebox{-0.92\totalheight}[0pt][\totalheight]
        {\includegraphics[width=0.4\columnwidth]{figures/mulhern.png}} & Anne Mulhern is a software engineer at Red Hat, Inc. She has been writing software projects in Rust since 2016. Her research interests are motivated by the practical problems she encounters in her day to day work. She has contributed to a variety of open-source software projects and presented at several open-source conferences. Before she joined Red Hat she worked as a professor at a number of colleges and universities in the United States. She received her Ph.D. in Computer Sciences from the University of Wisconsin-Madison. \\
        \raisebox{-0.92\totalheight}[0pt][\totalheight]
        {\includegraphics[width=0.4\columnwidth]{figures/sanjay.jpg}} & Sanjay Arora is a research scientist at Red Hat Research and works on applying machine learning to optimize low-level systems. \\
        \raisebox{-0.92\totalheight}[0pt][\totalheight]{\includegraphics[width=0.4\columnwidth]{figures/rayb.png}} & Baishakhi Ray is an Associate Professor in the Department of Computer Science at Columbia University, NY, USA. She has received the prestigious IEEE TCSE Rising star award and NSF CAREER award. Baishakhi’s research interest is in the intersection of Software Engineering and Machine Learning. Her research has been acknowledged by many Distinguished Paper awards and has also been published in CACM Research Highlights.
    \end{tabular}
\end{table}

==> sections/intro_back.tex <==
\section{Introduction}

The \rust programming language is gaining increasing popularity among systems programmers for its efficient performance while providing strong memory safety, thread safety, and type checking. It uses a C-like syntax that allows low-level access, enabling it to be used on embedded devices, to write kernel code, to build performance-critical systems, and so on. At the same time, it ameliorates many of the pitfalls of C, like pointer errors and concurrency errors. For these reasons, Google recently extended support for developing the Android OS in \rust \cite{google-2021a}, and has been pushing to include \rust in the Linux kernel \cite{google-2021b}. Linus Torvalds, the lead developer of the Linux kernel, recently said that \rust will be supported in the next kernel release \cite{vaughan-nichols-2022}.

Despite the strong safety guarantees promised by \rust, an increasing number of security vulnerabilities (CVEs) have been reported in \rust projects. The number of CVEs reported to the RUSTSEC Database \cite{rustsec} during 2018 was only 22; by 2021, the number is increased to 144. The majority of these CVEs arise from the use of a language feature called \TT{unsafe} \rust \cite{xu2020memory}---\rust's memory safety guarantees can be too restrictive for some applications, so \rust provides an ``escape hatch'' in the form of \TT{unsafe} \rust, which allows writing code that bypasses some %of \rust's 
memory safety checks.
The added flexibility comes at the cost of potential memory safety errors. 

Thus, while using \TT{unsafe} \rust, it is the developer's responsibility to ensure the code is correct---a single mistake may jeopardize the whole \rust program's safety guarantee and inadvertently introduce vulnerability in the program. To this end, this paper introduces a novel static analysis tool designed to assist developers in checking memory usage correctness within unsafe \rust code, thereby detecting potential violations. 

\smallskip
\noindent
\textbf{\rust memory safety model.} While working within the secure confines of \rust, we enjoy robust safety guarantees. 
Central to these assurances is \rust's \textit{Ownership} model\textemdash a set of rules dictating memory management within a \rust program. 
Ownership guarantees that a memory location is owned by exactly one identifier at any instant during program execution. Most modern programming languages handle memory usage during execution in some way or other---with some relying on garbage collection (e.g., Java) and others on manual allocation and deallocation (e.g., C). \rust takes an alternative approach with the concept of ownership, reinforced by a specific set of compiler-verified rules. Any violation of these rules results in a compilation failure. However, none of the ownership features affect the \rust program with run-time slowdowns.






% One of the key features \rust provides to protect against memory errors are 
%We now briefly discuss some features of \rust, to lay the foundation for the techniques we present in this paper. Two key concepts in \rust are 
%To protect against memory errors, \rust has some inbuilt features. 
% Nevertheless, if we stay within the framework of safe \rust, we have strong safety guarantees. 
% A key feature of \rust that contributes to these guarantees is its \textit{Ownership} model. 
% Ownership refers to a set of rules that dictate how a \rust program will manage its memory. 
% Modern programming languages handle memory usage during their execution---while some languages like Java rely on garbage collection to reclaim unused memory, others like C/C++ require manual allocation and deallocation by the programmer. Rust, however, adopts a third approach by using the concept of ownership with a specific set of rules that are verified by the compiler. Should any of these rules be breached, the program will fail to compile. Importantly, none of the ownership features impose runtime slowdown on your program.

%Rust employs an ownership system with compiler-verified rules to manage memory in programs. 
%Unlike languages using garbage collection or manual allocation, Rust ensures memory safety by halting compilation when ownership rules are violated. Importantly, these ownership features do not add any runtime performance overhead to your program.

%\rust's most distinctive attribute is ownership, which holds profound ramifications for the entire language. 
%The ownership concept empowers \rust to ensure memory safety effectively, all while circumventing the necessity for a garbage collector.

%A key feature of Rust that contributes to these guarantees is its \textit{Ownership} model. 

The strict ownership policy of one memory location owned by only one identifier at any given time, are often overly limiting. Thus, \rust allows \textit{Borrowing}---
%A memory location is owned by exactly one identifier at any instant during program execution. 
another identifier may temporarily borrow a memory location under certain conditions.

Every identifier has assigned to it by the compiler a \textit{Lifetime}, that is, a region of the source code in which the identifier is live. Unlike the more familiar \textit{scope}, the lifetime of a \rust identifier is not determined by an obvious lexical marker like a pair of braces but may terminate at any statement.

When an owning identifier ceases to be live, its corresponding memory location is released, avoiding memory leaks. \rust must ensure that no borrowing identifier can be dereferenced after the memory has been released. To ensure this property holds for all \rust programs is the responsibility of the \textit{Borrow Checker}

The Borrow Checker must assign to every identifier a lifetime that satisfies the above requirement and all other semantics of the program. Often the Borrow Checker can infer the lifetime of an identifier without assistance. In other cases, however, the Borrow Checker requires that \textit{lifetime annotations} be inserted in the source code to guide the Borrow Checker.




The system of Ownership, Borrowing, and Lifetimes is intended to provide strong memory safety guarantees to \rust. However, the \rust Borrow Checker is based on static program analysis, and determining the lifetime of each identifier statically is an undecidable problem \cite{landi1992undecidability}. So the Borrow Checker makes a deliberate approximation to be \textit{conservative} in its analysis: it is better to reject \textit{some} valid programs than allow \textit{any} invalid programs.

\textbf{Unsafe \rust.}
If a developer is sufficiently constrained by the restrictions of safe \rust, unsafe \rust, which is an extension of safe \rust may provide the required expressiveness. Unsafe \rust allows a few additional operations and declarations prohibited in safe \rust, including dereferencing raw pointers. Unsafe code is delimited in \rust with the \TT{unsafe} keyword.

When using unsafe code, i.e., code marked by the \TT{unsafe} keyword, it is the responsibility of the developer to ensure that the use is correct. In particular, if defining a safe function that uses unsafe \rust, for example, by invoking another function marked unsafe, the developer must ensure that the calling function is actually safe, i.e., that it satisfies all the expected properties of safe \rust. A significant part of this challenge is that of selecting correct lifetime annotations for such functions. A one-character mistake in specifying correct lifetime annotations can lead to security vulnerabilities, as we see from a manual inspection of reported \rust CVEs. In this paper, we focus on automatically detecting such \textit{incorrect lifetime annotations}.

\textbf{Limitation of Existing Approaches.} Checking the safety of unsafe \rust is an active area of research, with multiple reported vulnerabilities \cite{rustsec, xu2020memory}, and automated tools that perform static \cite{bae2021rudra, li2021mirchecker, cui2021safedrop}, and dynamic \cite{miri, cargofuzz} analysis to check for vulnerabilities. However, none of these existing tools can detect memory-safety bugs due to incorrect lifetime annotations. %, which is one of the leading causes of security vulnerabilities listed in CVEs.

\textbf{Our approach:} 
In this paper, we propose a lightweight static analysis technique, \sysname{},  that can automatically scan a \rust project and look for potential lifetime annotation errors. To do that, we first define three error patterns based on types of operations involving a raw pointer and a borrow.
\be
 \item \textbf{\textsc{Get}:} Return a borrow to the value pointed to by the raw pointer.
 \item \textbf{\textsc{Set}:} Update the raw pointer to point to a borrowed value.
 \item \textbf{\textsc{Create}:} Use a borrowed value to create a new structure object with a raw pointer.
\ee
% \rayb{add one lines for each three patterns}

\sysname{} first looks for structures and methods that deal with raw pointers and searches for function signatures matching our error patterns. Then it performs a lightweight taint analysis to trace the connections between borrows and raw pointers. The approximate analysis of  \sysname{} makes it possible to scale effortlessly to detect errors across multiple large \rust projects.



% In this paper, we investigate a specific type of error in \TT{unsafe} \rust: errors caused by \textit{incorrect lifetime annotations} on borrows. Our \textit{key insight} is that lifetime annotations guide the borrow checker in determining how long a borrow can live, and incorrect annotations on borrows could lead to memory safety bugs. We focus our analysis on borrows occurring in a very specific setting. Consider structures containing raw pointers (pointers that are not tracked by the Borrow Checker). These structures usually have methods (functions) that manipulate the raw pointers within them. Our analysis focuses only on borrows that are \textit{arguments} of, or \textit{returned} by, such functions.

% We first identify and define three possible patterns of bugs arising from incorrect lifetime annotations in our chosen setting. These correspond to the different kinds of operations that a function can perform with a borrow. We show that these bug patterns are a cause of vulnerabilities in \rust projects by manually inspecting the list of all reported \rust CVEs.

% Motivated by our manual study, we propose \sysname{}, a tool based on static analysis that can automatically scan a \rust project and look for the three bug patterns that we defined. \sysname{} first looks for structures and methods that handle raw pointers, and searches for function signatures matching our error patterns. Then it performs a lightweight taint analysis to trace the connections between borrows and raw pointers. \sysname{} is built to scale effortlessly to detect errors in multiple large \rust projects.

\textbf{Summary of results:}
We perform the following experiments.
\be
\item We evaluate \sysname{} on packages from the \rust package registry, and find 6 new bugs. 
%Overall \sysname{} detected 26 bugs with 46\% false positive rate.
%with a false discovery rate of 46\%.
\item Further, we run \sysname{} on 4 CVEs that we identify as arising from incorrect lifetime annotations, and find that it is able to correctly flag 3 out of 4 as bugs.
\item We run existing static analysis approaches on a) 3 hand-crafted toy examples, b) the 6 bugs we found, c) the 4 CVEs we identified. We show that they are unable to detect \textit{any} of these bugs.
\ee

\textbf{Contributions:} Our contributions in this paper are as follows.
\be
\item We investigate the mechanisms by which incorrect lifetime annotations can lead to memory safety bugs, and create a taxonomy of three patterns of bugs.
\item We perform a manual study of \rust security vulnerabilities (CVEs) to identify those arising from incorrect lifetime annotations. Further, we classify each of these vulnerabilities according to our taxonomy of bugs.
\item We propose \sysname{}, a static analysis based tool that can automatically scan \rust projects and detect potential errors caused by incorrect lifetime annotations. We evaluate \sysname{} on real-world \rust projects and show that it is able to successfully detect errors.
\ee

To the best of our knowledge, \sysname{} is the first static analysis tool that can analyse the lifetime annotations in \rust projects at scale and detect potential errors. We hope that our tool will be an aid to \rust developers, and we make the code publicly available (anonymized for review) \footnote{\url{https://github.com/vnrst/Yuga}}.

The rest of the paper is structured as follows. In Section \ref{sec:background}, we discuss the features of \rust and lifetime annotations. Then, we define three patterns of lifetime annotation bugs in Section \ref{sec:patterns}. Section \ref{sec:methodology} presents the design of \sysname{}, our tool to detect lifetime annotations bugs. We evaluate the performance of \sysname{} in Section \ref{sec:rqs}, present related work in Section \ref{sec:related_work}, and conclude in Section \ref{sec:conclusion}.

% \rayb{add the structure of the paper.}

==> sections/intro_back2.tex <==
\section{Introduction}

The \rust programming language is gaining increasing popularity among systems programmers for its efficient performance while providing strong memory safety, thread safety, and type checking. It uses a C-like syntax that allows low-level access, enabling it to be used on embedded devices, to write kernel code, to build performance-critical systems, and so on. At the same time, it ameliorates many of the pitfalls of C, like pointer errors and concurrency errors. For these reasons, Google recently extended support for developing the Android OS in \rust \cite{google-2021a}, and \rust is officially supported in the Linux kernel as of Linux 6.1 \cite{vaughan-nichols-2022}.


\smallskip
\noindent
\textbf{\rust memory safety model.} While working within the secure confines of \rust, we enjoy robust safety guarantees.
Central to these assurances is \rust's \textit{Ownership} model\textemdash a set of rules dictating memory management within a \rust program. 
Ownership guarantees that each value and its associated memory are owned by exactly one identifier at any point in the program. Modern programming languages handle memory usage during execution in different ways---some rely on garbage collection (e.g., Java) and others on manual allocation and deallocation (e.g., C). \rust takes an alternative approach with the concept of ownership, reinforced by a specific set of compiler-verified rules. Any violation of these rules results in a compilation failure. Yet, none of these rules slow down the run-time of \rust programs.

However, the strict ownership policy---each value owned by only one identifier at any given time, is often overly limiting. Thus, \rust allows \textit{Borrowing}---another identifier may temporarily borrow a value under certain conditions by creating a reference to that value. Consider the statement \TT{a = \&b}, here \TT{a} is borrowing the value \TT{b}.
\rust further introduces the concept of \textit{Lifetimes} to restrict a borrow's scope---a lifetime is a region of the source code in which the borrowing identifier is live; the borrowing identifier must not outlive the borrowed value (\eg~  \TT{a} cannot outlive \TT{b} in the above example). 

The \rust compiler, specifically its \textit{Borrow Checker}, ensures the validity of all borrows by tracking variable lifetimes. Often the checker can infer the lifetime of a variable without assistance.
However, for certain cases related to inter-procedural reasoning, 
the compiler requires explicit \textit{lifetime annotations} on function signatures to guide the Borrow Checker. For example, the type \TT{\&'a i32} denotes a borrow to an integer value, where the lifetime of the borrow is 
parameterized by the lifetime annotation \TT{'a}.

These annotations on the function signature provide valuable information to the compiler, enabling it to verify certain memory safety properties without even looking at the function body.


\smallskip
\noindent
\textbf{Violation of memory safety guarantees.}
Despite the strong safety guarantees promised by \rust, an increasing number of security vulnerabilities have been reported in \rust projects. The number of vulnerabilities reported to the RUSTSEC Database \cite{rustsec} during 2018 was only 22; in 2022, there were 91. The majority of these vulnerabilities arise from the use of a language feature called \TT{unsafe} \rust \cite{xu2020memory}---\rust's memory safety guarantees can be too restrictive for some applications, so \rust provides an ``escape hatch'' in the form of \TT{unsafe} \rust, which allows writing code that bypasses some %of \rust's 
memory safety checks.
The added flexibility comes at the cost of potential memory safety-related bugs. 

Thus, while using \TT{unsafe} \rust, it is the developer's responsibility to ensure the code is correct---a single mistake may jeopardize the whole program's safety guarantees and inadvertently introduce vulnerability. One of the causes of such vulnerabilities is incorrect lifetime annotations (\las) on function signatures.

Deciding the correct \las for a variable is non-trivial---it requires expert knowledge of how the value will propagate to subsequent borrows and pointers, often through deeply nested structures and function calls. Further, lifetimes in \rust are a non-intuitive concept even for experienced programmers, as there is no analogous concept in any other popular programming language (to the best of our knowledge). A one-token mistake in specifying correct \las can lead to security vulnerabilities, as we see from a manual inspection of reported \rust security vulnerabilities\footnote{Here is one example: \url{https://github.com/rust-lang/futures-rs/pull/2206/files}}.


\textbf{Limitation of Existing Approaches.} Checking the safety of unsafe \rust is an active area of research, with multiple reported vulnerabilities \cite{rustsec, xu2020memory}, and automated tools that perform static \cite{bae2021rudra, li2021mirchecker, cui2021safedrop}, and dynamic \cite{miri, cargofuzz} analysis to check for vulnerabilities.
However, none of these existing tools can detect memory-safety bugs due to incorrect \las. 

First of all, \la-related bugs are rare and typically only surface during execution in specific edge cases. Thus, detecting them through dynamic analysis or testing is non-trivial. Additionally, they tend to be deeply embedded within a program, and analyzing them requires accurate modeling of program memory. Thus, it becomes challenging to study using standard static analyzers or symbolic execution tools. 
Even, more mature hybrid vulnerability detection tools designed for other languages like C/C++  cannot be applied here as \la is a new concept introduced in \rust.  
 

To this end, we propose a novel static analysis tool to check correct memory usage in unsafe \rust code. 
In particular, we focus on detecting incorrect lifetime annotations (\las) as they often lead to security vulnerabilities.

\textbf{Our approach:} 
We have developed and implemented a novel static analysis tool called \tool, capable of detecting incorrect \la bugs. 
We employ a multi-phase analysis approach that starts with a pattern-matching algorithm to quickly identify the potential buggy components. 
Subsequently, we perform a flow and field-sensitive alias analysis, focusing only on the potential buggy components to confirm the bugs. 
By adopting this multi-phase analysis, we effectively address the well-known scalability challenges associated with alias analysis, while still achieving reasonably high precision.



In particular, \tool operates in four stages. First, it propagates the LAs from a function parameter to internal references, pointers, and fields, using an AST-like representation. In the second stage, it identifies any potential mismatches in LAs between the function arguments and return values. These first two steps are challenging since they involve analyzing relationships between program variables through nested pointers and structures. When a mismatch is found, \tool flags the corresponding pairs of values as potentially buggy. 
Next, in the third stage, \tool conducts a flow and field-sensitive alias analysis to confirm the interactions between the source and target, further validating the presence of bugs. Up to this point, the analysis is intra-procedural. In the final stage, \tool employs specific shallow filters based on common inter-procedural analysis knowledge to reduce false positives, thereby improving the overall precision.

\textbf{Results.} We evaluate \tool using a dataset of known security vulnerabilities, and a synthesized vulnerability dataset. We find that \tool can detect \la bugs with 75\% precision. None of the existing static analysis tools we evaluated could detect \textit{any} of these vulnerabilities.
We also ran \tool on 2000 \rust libraries, and \tool detected 312 potential bugs. We are in the process of generating exploits of these bugs and reporting them to the developers.


\textbf{Contributions:} Overall contributions in this paper are as follows.
\be
\item We are the first to characterize incorrect lifetime annotations that can lead to memory safety bugs. 
\item We propose \sysname{}, a novel static analysis technique, that can automatically scan \rust projects at scale and detect potential \la bugs that can lead to vulnerabilities. 
\item We evaluate \sysname{} in a variety of settings and show that it can successfully detect \la bugs with good precision. 
To the best of our knowledge, there are no existing baseline static analyzers that can find these bugs. 

\item We contribute two new datasets of lifetime annotation bugs, one created from \rust security vulnerabilities, and the other synthetic.  We make the code and dataset publicly available (anonymized for review) \footnote{\url{https://github.com/vnrst/Yuga}}.

\ee


The rest of the paper is structured as follows. In~\Cref{sec:background}, we discuss the features of \rust and lifetime annotations. Then, we define three patterns of lifetime annotation bugs in~\Cref{sec:patterns}.~\Cref{sec:methodology} presents the design of \sysname{}, our tool to detect lifetime annotations bugs. We evaluate the performance of \sysname{} in~\Cref{sec:setup,sec:rqs}, present related work in~\Cref{sec:related_work}, and conclude in~\Cref{sec:conclusion}.

% \rayb{add the structure of the paper.}

==> tools/README <==

August 26, 2015


The IEEEtrantools.sty package provides several commands from the
IEEEtran.cls file so that they can be used under other LaTeX classes. The
user guide provided here covers only the differences in the use of the
commands from those provided by IEEEtran.cls. For complete documentation
on these commands, see the relevant sections in the IEEEtran_HOWTO manual
of the IEEEtran LaTeX class.

The IEEEtrantools.sty package provides the following IEEEtran.cls commands:

 1. \IEEEPARstart which produces large initial "drop cap" letters.

 2. The \bstctlcite command for the control entry types of IEEEtran.bst
    V1.00 and later.

 3. The \IEEEnoauxwrite command.

 4. The IEEE itemize, enumerate and description list environments.

 5. The complete IEEEeqnarray family for producing multiline equations
    as well as matrices and tables, including the IEEEeqnarray support
    commands.

 6. The \IEEEQEDhere and \IEEEQEDhereams commands to provide amsthm.sty
    \qedhere functionality to IEEEproof. \IEEEQEDhere is for simple use
    "right on the spot" such as within an IEEEeqnarry:

    \begin{IEEEproof}
       \begin{IEEEeqnarray}{rCl+x*}
        x & = & y & \nonumber\IEEEQEDhere
       \end{IEEEeqnarray}
    \end{IEEEproof}

    While \IEEEQEDhereams is like amsthm's venerable \qedhere and is
    for use within the standard equation environment:

    \begin{IEEEproof}
     \begin{equation}
       x = y \nonumber\IEEEQEDhereams\quad
     \end{equation}
    \end{IEEEproof}

    Note that the qedhere style is normally not done with IEEE-related
    work so these are undocumented features of IEEEtran.cls.

    Thanks Mark D. Butala, Hennadiy Leontyev and Stefan M. Moser for
    suggesting this feature.



IEEEtrantools.sty is not needed and should not be used with IEEEtran.cls.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtrantools support page at my website:

http://www.michaelshell.org/tex/ieeetran/tools/


Enjoy!

Michael Shell
http://www.michaelshell.org/


*******
2015/08/26 V1.5 (V1.8b of IEEEtran.cls) changes:

 1) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 2) Fix bug with IEEEeqnarray equation number foreground color
    under the color environment of Beamer class.
    Thanks to Joschi Brauchle for reporting this problem.

 3) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.



********************************** Files **********************************

README                - This file.

changelog.txt         - The revision history.

IEEEtrantools.sty     - The LaTeX package file.

IEEEtrantools_doc.txt - The user manual - supplementary to the 
                        IEEEtran_HOWTO manual.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtrantools.sty, IEEEtrantools_doc.txt
***************************************************************************


